A Comprehensive Modeling Approach for Crop Yield Forecasts using AI-based Methods and Crop Simulation Models

Numerous solutions for yield estimation are either based on data-driven models, or on crop-simulation models (CSMs). Researchers tend to build data-driven models using nationwide crop information databases provided by agencies such as the USDA. On the opposite side of the spectrum, CSMs require fine data that may be hard to generalize from a handful of fields. In this paper, we propose a comprehensive approach for yield forecasting that combines data-driven solutions, crop simulation models, and model surrogates to support multiple user-profiles and needs when dealing with crop management decision-making. To achieve this goal, we have developed a solution to calibrate CSMs at scale, a surrogate model of a CSM assuring faster execution, and a neural network-based approach that performs efficient risk assessment in such settings. Our data-driven modeling approach outperforms previous works with yield correlation predictions close to 91\%. The crop simulation modeling architecture achieved 6% error; the proposed crop simulation model surrogate performs predictions almost 100 times faster than the adopted crop simulator with similar accuracy levels.

==> Makefile <==
PWD = $(shell pwd)

TEXINPUTS = ${PWD}:
BSTINPUTS = ${PWD}:

SETENVVAR = \
			BSTINPUTS="${BSTINPUTS}" \
			TEXINPUTS="${TEXINPUTS}"

SOURCE_FILES = $(wildcard *.tex *.bib)

BIBTEX = ${SETENVVAR} bibtex
LATEXMK = ${SETENVVAR} latexmk
PDFLATEX = ${SETENVVAR} pdflatex -shell-escape --synctex=1

.PHONY: clean

all: paper.pdf

paper.pdf: ${SOURCE_FILES}
	${PDFLATEX} paper.tex
	${BIBTEX} paper
	latex_count=6 ; \
	while egrep -s 'Rerun (LaTeX|to get cross-references right)' paper.log && [ $$latex_count -gt 0 ] ;\
		do \
			echo "Rerunning latex..." ;\
			${PDFLATEX} paper.tex ;\
			latex_count=`expr $$latex_count - 1` ;\
		done
	${BIBTEX} paper
	${PDFLATEX} paper.tex


clean:
	rm -f *.aux *.auxlock *.dvi *.lof *.lot *.lox *.toc *.bbl *.blg *.blf *.pyc *.bak *.log *.out *.fls *.fdb_latexmk *_latexmk *.synctex.gz paper.pdf


==> experiments.tex <==
\section{Experiments}\label{sec:experiments}

\begin{table}[h]
	\centering
  \scriptsize
	\begin{tabular}{lccc}
		\toprule
		Model & Culture & Correlation & MAPE \\
		\midrule
		\citet{cunha2020estimating} & Soybean & 0.300 & 16.015 \\
		Ours & Soybean & \textbf{0.453} & \textbf{13.010} \\
		\midrule \\
		\citet{cunha2020estimating} & Corn & 0.881 & 47.855 \\
		Ours & Corn & \textbf{0.912} & \textbf{43.063} \\
		\bottomrule
	\end{tabular}
	\caption{
		Comparison of results between previous and current model
		for Soybean and Corn crops in Brazil for 2018. Values
		in bold designate better performance.
	}\label{tab:nn-results}
\end{table}

\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{notebooks/uncertainty-Corn.pdf}
  \caption{%
    Yield estimates for corn in Brazil for 2018. Predictions are improved
    by having an associated uncertainty level represented by standard deviation.
    As can be seen in the graph, most extreme standard deviation values are
    also the ones with higher associated error.
  }\label{fig:nn-yield}
\end{figure}

%Trial 3 finished with value: -0.9143439061315815 and parameters: {'entropy': 0.4315156597167873, 'noise': 0.11959567881555487}. Best is trial 3 with value: -0.9143439061315815.
%
%{'Correlation': 0.9143439061315815,

This section presents experiments and their underlying results considering the
three proposed modeling approaches (Figure~\ref{fig:methodology}). With this
experiment set, we demonstrate the feasibility of our proposed solution by
estimating soybean and corn yield for Brazil and soybean in Illinois with
data-driven and crop simulation model solutions respectively. Although we show
results related to soybean and corn for Brazil and the USA, our approach is
generic enough to consider other crops and regions as we did in previous work
in which we evaluated soybean, corn, rice, sugarcane, and
cotton~\cite{oliveira2018scalable,cunha2020estimating}.

Initially, we evaluate soybean and corn yield for Brazil in 2018 and compare it with
previous work. Next, we investigate how crop simulation models can be used to
assess soybean production for several years in Illinois-USA with multiple
calibration ensembles. Finally, we show how surrogates can perform
fast-assessment of crop simulation models without running the actual model.

\begin{figure}
	\centering
	\input{notebooks/reliability-plots.tex}
	\caption{%
		Calibration~\citep{kuleshov2018accurate} plots for both trained models.
		Both models were trained and evaluated independently, with new
		noise and entropy hyperparameters optimized independently, but sharing
		others, such as number of epochs, learning rate, and early stopping
		patience.
	}\label{fig:calibration}
\end{figure}

\subsection{Data-Driven Model Results}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{img/CombinedResults.pdf}
    \caption{
        Crop simulation model results using different calibration ensembles. 
    }\label{fig:csm_results}
\end{figure*}



Here we describe results obtained when we apply to our model the improvements
described in the Section~\ref{sec:neural-network}. We show that not only our
estimates are better than with point estimates, but also that uncertainty
information is useful to interpret the output of the model.

% TODO: Add actual link. Here we compare the results of the new model with We
We compared the results from our previous work~\citep{cunha2020estimating} for
estimation of Soybean productivity in Brazil for 2018 and followed the same
training procedure used there with the same model setup and hyperparameters.
For the hyperparameters introduced in this paper (noise and entropy
regularization), we performed 66 trials of hyperparameter optimization with
Optuna~\cite{optuna_2019}, which yielded noise = $0.0824$, and $\eta=0.2359$
for the soybean model, and noise = $0.0984$, and $\eta=0.3451$.
The other hyperparameters were: learning rate $\alpha=5\times10^{-4}$, maximum
number of epochs set to $1000$, with early stopping patience set to $50$.

In Table~\ref{tab:nn-results}, we see a summary of the results for soybeans
and corn. As can be seen, the neural network yields more accurate results
than the previous iteration, \emph{while also providing uncertainty
information}. Uncertainty information is highlighted for Corn in
Figure~\ref{fig:nn-yield}. As implied from the graph, higher uncertainty
predictions can have different treatment than predictions with less
uncertainty.

To assess whether the uncertainty estimates of the models are useful, we also
plotted calibration diagrams~\citep{kuleshov2018accurate}\footnote{
	Not to be confused with the calibration process of simulation models,
	presented in the next section.
} for both models.
Calibration means that a predicted value $y_i$ should fall in a X\%
confidence interval X\% of the time. Formally, when $x_i, y_i$ are independent,
identically-distributed realizations of random variables $X, Y$, calibration
can be computed by
\begin{equation*}
	P(Y\le F_X^{-1}(p)) = p \text{ for all } p \in [0, 1]\text{,}
\end{equation*}
where $F_X$ is the forecast value at $X$. The calibration plots are shown in
Figure~\ref{fig:calibration}, and we can see that both trained models are close
to the ideal identity line, although the confidence expressed by the corn model
is smaller than it could have been, especially for larger confidence levels.

\subsection{Crop Simulation Model Results}

In this experiment, we study how soybean yield can be predicted using the
proposed crop simulation model service for Illinois (USA) counties in the
2010 to 2018 period. This section presents county-level
soybean predictions, however, the proposed approach is general enough to
calibrate and evaluate other crops data at farms level. For this study, we
selected 50 pixels at random using CropScape~\cite{han2012cropscape} data to
identify soybean fields. We also employed Quick Stats~\cite{nass2011quick}
service to obtain the measured yield for each county at a given year.
We evaluated the different ways of calibrated models ensemble presented in
Section~\ref{sec:evaluation}.

Figure~\ref{fig:csm_results} and Table~\ref{table:csv_results1} shows the
results for different ways of using calibrated models using previous seasons
data. Figure~\ref{fig:csm_results}a) shows the yield estimation results for
all possible combinations of calibrated model and further evaluation in later
years. This utilization of previously calibrated model is pretty simple and
provides less accurate results as it does not leverage multiple calibrated
models when performing crop yield estimation. For each evaluation, we present
in Figure the mean value as the predicted value. The system calculates the
standard deviation using all the predictions for the 50 pixels calibrated
within the county for a single year.

Figure~\ref{fig:csm_results}b) depicts the results when we compare the
measured yield and the mean value of the previous calibrated models. Observe
that using the model calibrated in the last year improves the ensemble
performance. The results suggest a strong correlation between the close
planting years. One can explain this fact as farming management procedures,
and even climate change effects usually take time to change.
This hypothesis gets stronger when we observe the results considering the
mean value of previously calibrated years (Figure~\ref{fig:csm_results}c)).
In this case, the contribution to the final yield prediction of far
calibrated models is the same as close calibrated years. Observe the results,
in this case, are poor when compared to the previous calibrated year but
better than the simplest approach.

Although the previous approaches present quite good results, they can be
improved by using the other strategies to reduce the evaluation error. For
instance, as long as we use the proposed system during different years, we
can observe which calibrated model presents better predictions when compared
to others in different years. We can use a quality metric (MAPE) using
previous evaluation years to estimate how good a calibrated model tends to
perform and give more importance to this model (quality-based ensemble
strategy). Figure~\ref{fig:csm_results}d) shows the better prediction
results we found in this study as it gives more weight to calibrated models
that perform well previously. Observe this ensemble generates a higher 
standard deviation as it attributes different weights to previous calibrated
models increasing prediction variability for each pixel.

The results shown in Figure~\ref{fig:csm_results}d) considers all the
evaluation years in the study interval. However, crop yield evaluation years
should have different numbers of calibration model sizes to create theirs
ensembles. For instance, 2012 has more calibrated models to create its
ensemble than all the others. Figure~\ref{fig:erros_time} shows how evaluation
errors change according to the number of previous calibrated years, observe 
there is performance increase pattern when there is a higher number of previously
calibrated models. 

\begin{table}
	\centering
  \scriptsize
\begin{tabular}{cccc}
\toprule
                    Experiment &  Correlation &      MAPE &     RMSEP \\
\midrule
        All previous calibrations &  0.580 &  0.146 &  0.180 \\
        Previous calibrated year &   0.705 &  0.125 &  0.144 \\
    Mean of previous calibrations &  0.669 &  0.132 &  0.150 \\
        Quality-based ensemble &     0.747 &  0.113 &  0.130 \\
\bottomrule
\end{tabular}
\caption{
    Performance metrics for different calibration ensembles.
}
\label{table:csv_results1}
\end{table}


\begin{figure}[h]
  \centering
  \includegraphics[width= .99\linewidth]{img/errors.pdf}
  \caption{%
  Error-related metrics for the quality-based ensemble for calibrated for
  different years. Observe the model performance tends to improve as the
  number of years increases.
  }\label{fig:erros_time}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Indicate the infrasctructure used to evaluate the CSM
% It takes one day to calibrate and 2 days to evaluate
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Crop Simulation Model Surrogate Results}

A surrogate model can be considered a good one if it is be able to replicate
similar results of the target model, with reduced computational time. On
total, we have generated 700 different combinations of parameters with the
Saltelli sampling strategy, and the associated yield calculated by DSSAT. We
have user 75\% of this dataset as the training set, using the remaining 25\%
as the test set for validation purposes. Our approach with NN achieved
satisfactory results, presenting an average $R^2$ correlation on the training
dataset equal to $0.96$ (obtained from 5 rounds of execution), and an evident
computational time reduction. To execute DSSAT for the training and test
datasets ($700$ entries on total), it was required on average 2 min to complete
the task on a 16-core cluster with $256$GB RAM. On the other hand, for
predicting the test dataset ($135$ entries), it required a single core
processor with RAM $16$Gb memory and less than a second for execution. It is
clear that regarding time and computational consumption there was a clear
improvement with the usage of the surrogate model.

\begin{figure}
  \centering
  \includegraphics[width=.99\linewidth]{img/surrogate_nn_dssat.pdf}
  \caption{%
    Yield estimates for soybean in Brazil for 2018. Predictions are improved
    by having an associated uncertainty level represented by standard deviation.
    As can be seen in the graph, most extreme standard deviation values are
    also the ones with higher associated error.
    }\label{fig:nn-dssat}
\end{figure}

The high accuracy in the prediction provided by the NN can indicate a possible
overfitting of data, which would demand the validation with a totally different
test set. The test set was composed by a random entries generated by the
Saltelli method over a specified range of each parameter. So, it very likely
that each sample from the test set presented a very close entry used in the
training phase. It indicates, however, that performing an extensive and
efficient sampling of the parameters space to generate artificial data for the
construction of a NN is promising. If we can cover reasonably well the whole
parameter space for the construction of the surrogate model, chances as high
that a new entrance is somehow close to one instance in the training set. In
this sense, the use of the Saltelli method for sampling seems to be the best
option, as it mix random samples and guided samples to unexplored areas of the
search space.

